Efficient GNN Training Through Structure-Aware Randomized Mini-Batching

Graph Neural Networks (GNNs) enable learning on realworld graphs and mini-batch training has emerged as the de facto standard for training GNNs because it can scale to very large graphs and improve convergence. Current mini-batch construction policies largely ignore efficiency considerations of GNN training. Specifically, existing mini-batching techniques employ randomization schemes to improve accuracy and convergence. However, these randomization schemes are often agnostic to the structural properties of the graph (for eg. community structure), resulting in highly irregular memory access patterns during GNN training that make suboptimal use of on-chip GPU caches. On the other hand, while deterministic mini-batching based solely on graph structure delivers fast runtime performance, the lack of randomness compromises both the final model accuracy and training convergence speed. In this paper, we present Community-structure-aware Randomized Mini-batching (COMM-RAND), a novel methodology that bridges the gap between the above extremes. COMM-RAND allows practitioners to explore the space between pure randomness and pure graph structural awareness during mini-batch construction, leading to significantly more efficient GNN training with similar accuracy. We evaluated COMM-RAND across four popular graph learning benchmarks. COMM-RAND cuts down GNN training time by up to 2.76x (1.8x on average) while achieving an accuracy that is within 1.79% points (0.42% on average) compared to popular random mini-batching approaches.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> abstract.tex <==
\begin{abstract}

%Graph Neural Networks (GNNs) enable learning on real-world graphs and power critical applications such as social network analysis, traffic forecasting, and anomaly detection.
Graph Neural Networks (GNNs) enable learning on real-world graphs and mini-batch training has emerged as the de facto standard for training GNNs because it can scale to very large graphs and improve convergence. 
Current mini-batch construction policies largely ignore efficiency considerations of GNN training.
Specifically, existing mini-batching techniques employ randomization schemes to improve accuracy and convergence. 
However, these randomization schemes are often agnostic to the structural properties of the graph (for eg. community structure), resulting in highly irregular memory access patterns during GNN training that make sub-optimal use of on-chip GPU caches. 
On the other hand, while deterministic mini-batching based solely on graph structure delivers fast runtime performance, the lack of randomness compromises both the final model accuracy and training convergence speed.
In this paper, we present \emph{\underline{Comm}unity-structure-aware \underline{Rand}omized Mini-batching} (\sysname), a novel methodology that bridges the gap between the above extremes.
\sysname allows practitioners to explore the space between pure randomness and pure graph structural awareness during mini-batch construction, leading to significantly more efficient GNN training with similar accuracy.
We evaluated \sysname across four popular graph-learning benchmarks. \sysname cuts down GNN training time by up to 2.76x (1.8x on average) while achieving an accuracy that is within 1.79\% points (0.42\% on average) compared to popular random mini-batching approaches.   
%%

%Graph Neural Networks (GNNs) have emerged as the de facto standard for analyzing massive graphs such as social networks, but efficiently processing graphs with millions of nodes and edges remains a significant challenge. While mini-batching is commonly employed to address this limitation, current mini-batch construction policies largely ignore performance considerations. Specifically, \haggai{consider marketing the following points as a contribution of ours achieved via experiments} uniform random mini-batching policies, while beneficial for accuracy and convergence, often degrade runtime performance as they tend to have inefficient memory access patterns. \christos{add half a sentence someplace around here about which HW features underperform with uniform random; where does the performance diff stem from} Conversely, purely deterministic approaches optimized for runtime performance can lead to reduced accuracy and slower convergence. 
%In this paper, we present \emph{\underline{Gra}ph-Structure-aware \underline{Rand}omized Mini-batching (GRAND)}, a novel methodology that bridges this gap through two innovations applied to key steps in the mini batching procedure: (1) incorporating graph structure-aware randomness in root node ordering, and (2) controlling structural bias in neighborhood sampling of these root nodes. This approach enables practitioners to explore the interplay between pure randomness and pure structural awareness, leading to more efficient training (almost) without sacrificing accuracy.
%Through extensive evaluation of four large-scale graph learning benchmarks, we demonstrate that GRAND achieves up to 2X improvement in runtime performance while maintaining comparable accuracy to existing approaches.
\end{abstract}


==> background.tex <==
\section{Background and prior work} \label{sec:background}
%\haggai{rewrote the bullet points. This section is not ready yet and needs work. there are several things we say here: (1) mini batching + randomization is what people currently use for training large graphs; (2) explain mini batching + algo box; (3) talk about graph aware reordering in GNNs in both training and inference. I am not sure the order in which it is currently written is optimal, and also not sure about the "background" title - it is not only background - we have some experimental evaluations there... }
%\VB{Tried breaking the contents into two sections -- "Background on GNN training" and "Randomization vs Graph-Structure". (Commented the existing text here as we work on spreading the content across 2 sections)}

We first provide a background on GNN training and discuss the difference between full-batch vs mini-batch training.
% 
After demonstrating the superiority of mini-batch GNN training, we provide a high-level overview of prior work on mini-batch construction.
%%


%% The purpose of this section is to establish mini-batch training as the baseline. We do it in 3 parts
%% \begin{itemize}
%%     \item (Mathematically) talk about full-batch vs mini-batch GNN training
%%     \item Show convergence results 
%%     \item Discuss prior work on mini-batch construction
%% \end{itemize}

{\bf Learning on graphs with GNNs:}
%
We focus on a common machine learning scenario in which the input consists of a single large graph and goal is to predict the attributes of individual nodes \cite{kipf2016semi}. A typical application is predicting the characteristics of users within a social network.
Consider a graph $G = (V, E)$ with $|V|$ nodes and $|E|$ edges. Its adjacency matrix $A$ has dimensions $|V| \times |V|$. Each node has an $F$-dimensional feature vector, with all node features collected in matrix $X \in R^{|V| \times F}$. In each layer of the graph neural network, a node's embedding is computed using the embeddings of its neighbors from the previous layer using the following update steps:
\begin{equation} \label{eq:gnn-embedding}
X^{l+1} = \sigma(A'X^{l}W^{l}), \quad l=1,\dots,L-1
\end{equation}
Here, $L-1$ is the number of GNN layers in the model, $X^{l+1}$ contains the embeddings of all nodes after layer $l$, $A'$ is the normalized and regularized adjacency matrix, $W^1,\dots, W^{L-1}$ are weight matrices and $\sigma$ is a pointwise non-linearity such as a ReLU function \footnote{Equation \ref{eq:gnn-embedding} is formulated using GCN layers \cite{kipf2016semi} without bias for simplicity, the formulation with other message passing neural networks is similar, see for example \cite{hamilton2017inductive}}.
 %
The goal of training is to learn the layer parameters $W^1,\dots,W^{L-1}$ by minimizing the loss between the labels of all labeled nodes and the node embeddings of the last layer. 
%
We refer readers to \cite{chiang2019cluster} for more detailed analysis time and space complexity of GNN training methods. 

{\bf Full-batch training:}
%
One of the earliest GNNs proposed was Graph Convolution Network (GCN) which used full-batch gradient descent for training~\cite{kipf2016semi}, i.e., propagating information through the entire graph simultaneously in every epoch.
%
Although full-batch training offers fast per-epoch processing times (by virtue of only updating gradients once every epoch and better utilization of GPU resources), full-batch needs to store all the intermediate embeddings for all nodes and layers.
%
Full-batch training of an $L$ layer GNN with $F$-dimensional feature vectors requires a memory footprint of $O(|V|FL)$ which makes scaling to large graphs infeasible.
%

\textbf{Mini-batch training:} An alternative to full-batch training is to perform mini-batch gradient descent where the basic unit of computation is a much smaller subset of nodes and the memory footprint reduces to $O(Bd^{L}F)$ where $B$ is the batch size and $d$ is the average degree of the graph.
%
To further reduce footprint, GraphSAGE~\cite{hamilton2017inductive} pioneered the concept of sampling the neighbors and bounding the maximum number of neighbors used for each node to $r$ further reducing the footprint to $O(Br^{L}F)$.
%%

\textbf{Superiority of mini-batch training:} Even on GPUs with sufficient memory capacity, mini-batch training is still preferable over full-batch training because mini-batch training makes gradient updates multiple times each epoch (once for every batch) and, therefore, converges in fewer epochs.
%
Our evaluation on the A100 GPU (80GB memory) across the {\tt reddit}, {\tt ogbn-products}, and {\tt igb-small} datasets (Section~\ref{sec:methodology}), shows that mini-batch training requires on average 10.2x fewer epochs to converge than full-batch training.
%
Consequently, mini-batch training is still 2.7x faster on total training time compared to full-batch training despite the latter having faster per-epoch processing times.
%
Therefore, beyond improved scalability, mini-batching's randomization enables faster convergence than full-batch training. Hence, we focus on randomized mini-batch training in this work.
%%
%% Therefore, due to its superior scalability and convergence behavior, we use mini-batch training as the baseline for our work.  
%%

{\bf Mini-batches construction techniques:} 
%
Algorithm~\ref{alg:minibatch} shows a typical mini-batch GNN training pipeline.
%
Mini-batch construction is a two-step process.
%
First, we need to divide the nodes in the training set across different batches.
%
The nodes within each mini-batch are also known as the root nodes and, hence, we refer to this step as root node partitioning (Line 2).
%
The second step constructs a sub-graph for each batch. 
%
Constructing the sub-graph involves traversing the $L$-hop neighborhood from all of the root nodes within the batch and then sampling a subset of those neighbors (Line 4).
%
All root nodes, sampled neighbors, and connections between them form the sub-graph of a specific batch.
%
The training computations (forward and backward passes) are performed on the sub-graphs (Line 6).
%
Specifically, the model takes in input features corresponding to the nodes within a batch's subgraph and then creates predictions. These predictions are then compared against the labels (corresponding to the root nodes in the batch) for the backward pass.
%% 

\begin{algorithm}[ht]
\caption{Mini-batch Training of an $L$-layer GNN}
\label{alg:minibatch}
\begin{algorithmic}[1]
\For{each training epoch}
    \State {\bf Step-1: Root node partitioning}
    \Statex \qquad Shuffle node IDs in training set $\bigstar$
    \Statex \qquad Divide nodes across mini-batches $\{B_1,...,B_k\}$
    \For{each mini-batch $B_i$}
        \State {\bf Step-2: Sub-graph Construction}
        \Statex \qquad \qquad Find $L$-hop neighbors of root nodes in $B_i$
        \Statex \qquad \qquad Sample a subset of the neighbors $\bigstar$
        \Statex \qquad \qquad Build sub-graph $S_i$ out of root nodes and sampled neighbors
        
    \EndFor
    \State Train on sub-graphs $\{S_1,...,S_k\}$
\EndFor
\end{algorithmic}
\end{algorithm}

GraphSAGE \cite{hamilton2017inductive} popularized the use of uniform randomization for both mapping root nodes across batches and sampling neighbors for the sub-graph construction.
%
Specifically, GraphSAGE performs uniform random shuffling of nodes in the training set (star under Line-2 in Algorithm~\ref{alg:minibatch}) and uniform random sampling of the $L$-hop neighborhood (star under Line-4).
%
The rationale for randomization every epoch is to expose the model to a broad range of nodes in the graph and produce diverse mini-batches that connect disparate regions of the graph for better generalization and convergence.
%
However, a problem with GraphSAGE is that the number of neighbors sampled grows exponentially with each extra layer (known as the {\em neighborhood explosion problem}).
%

To address the neighborhood explosion problem, various alternatives to mini-batch construction have been proposed (Liu et al. \cite{liu2021sampling} provide a comprehensive survey of GNN mini-batching techniques).
%
FastGCN~\cite{chen2018fastgcn}, LADIES~\cite{ladies}, and LABOR~\cite{labor} all use variations of importance sampling to sample fewer neighbors and bound the size of batches' sub-graphs.
%
ClusterGCN~\cite{chiang2019cluster} first partitions the graph and then builds mini-batches by randomly combining different partitions.
%
A common theme among all these prior mini-batch construction schemes is the use of randomization for achieving good accuracy and convergence with GNN training.
%
However, with the exception of clusterGCN, the randomization schemes are agnostic to graph structural properties which limits the ability to improve GNN training speed.
%
ClusterGCN, while a step in the right direction, suffers from limitations due to poor scalability with small training set sizes.
%
Section~\ref{subsec:prior-work-comparison} provides a quantitative comparison of the above prior work.
%%

%%In the next section, we discuss the ramifications of graph structure-agnostic randomization on the accuracy, convergence, and runtime performance of GNN training (Section~\ref{subsec:prior-work-comparison} shows a quantitative comparison of the above mini-batch construction techniques).
%%


%\haggai{This could be used here or moved to the prev work section. The pioneering work of Hamilton et al. \cite{hamilton2017inductive} introduced sampling techniques for processing large graphs with GNNs. Following the classical Graph Convolutional Network architecture \cite{kipf2016semi}, several works proposed efficiency improvements. Notable examples include ClusterGCN \cite{chiang2019cluster}, which employs graph partitioning algorithms to train the model on independent subgraphs, and FastGCN \cite{chen2018fastgcn}, which leverages importance sampling. However, the fundamental tradeoff between the level of randomness in minibatch generation and the degree to which sampled graphs preserve structural properties remains largely unexplored. To the best of our knowledge, no existing method allows for systematic tuning of structural bias and randomness levels in GNN minibatch construction.} \VB{I couldnt decide whether a discussion on related works belongs here, in the next section, or much later. For now, I tried to provide a brief insight into alternative mini-batch construction techniques with a forward pointer to more detailed (quantitative) analysis of the different techniques in the eval section}

%% \paragraph{Full-batch Training in GNNs.}
%% Training Graph Neural Networks (GNNs) on the entire graph at once eliminates the need for sampling techniques, avoiding any approximations or randomization in the training process. This approach provides exact gradient computations and deterministic updates to the model parameters. However, while conceptually simpler, full-batch training faces significant practical challenges as we discuss below. \footnote{While full-batch training has very high memory capacity requirements, we were actually able to run full-batch training on our medium-sized inputs on Ada RTX 6000 (48GB memory)}.
%% \paragraph{Mini-batch GNN Training.}
%% Mini-batch training is primarily used to reduce the memory footprint of GNN training by processing only a subset of nodes and their neighborhoods at any given time, instead of the entire graph. This approach introduces two key forms of randomization: data shuffling and neighborhood sampling. Algorithm~\ref{alg:minibatch} outlines the basic procedure.
%% The algorithm operates in three main phases. First, it creates mini-batches by randomly shuffling all node IDs and grouping them into smaller sets. Second, for each mini-batch of nodes, it constructs local subgraphs by sampling the $k$-hop neighborhoods around each node in the batch. This sampling is necessary as including complete neighborhoods could potentially span large portions of the graph, defeating the purpose of mini-batch training. Finally, the algorithm trains the GNN on these constructed subgraphs, updating the model parameters based on the computed gradients. This process repeats for each mini-batch, cycling through the entire graph over multiple epochs.


%% \paragraph{Empirical comparison.}
%% Our empirical analysis \haggai{add details here - which datasets, GPUs, and so on, do we have this only for one dataset? I think we probably need more to make a good point here} \christos{a forward pointer to the methodology section is also ok} reveals several key differences between full-batch and mini-batch training approaches:
%% \begin{enumerate}
%% \item \textbf{Convergence Speed:} Full-batch training requires significantly more epochs to converge, averaging 10x more epochs than mini-batch training.
%% \item \textbf{Model Accuracy:} Full-batch training achieves slightly lower final accuracy ($\sim$0.2 percentage points) compared to mini-batch training.
%% \item \textbf{Training Time:} Mini-batch training demonstrates a 2.72x speedup over full-batch training.
%% \end{enumerate}
%% Given these advantages in both scalability and convergence behavior, we adopt mini-batch training as the baseline approach in our work. \christos{earlier in the text you say that full batch training avoids approximations and provide gradient computations. This leads a reader to assume that FB training will be slow (or infeasible) but more accurate. So (1) and (2) from above are a little surprising. Provide some insights.}

%% \haggai{consider adding a background paragraph on memory and cache use to help ML people understand the big picture of how that works and why we see the what we see in the experiments.} \VB{Maybe we can provide some more details on caches when we talk about reordering in the next section?} \haggai{makes sense}

==> biased-rand.tex <==
\section{Biased Random Mini-batching} \label{sec:biased-rand}

%\christos{before you dive into details below, give readers a short overview of the ideas here. ~3 sentences. }
Uniform random mini-batching and entirely community-based mini-batching represent extreme points on the GNN training convergence vs per-epoch runtime trade-off space. 
%
The main contribution of our work is to explore the intermediate points of the trade-off space using {\em community structure-aware randomization} (\sysname) for mini-batch construction.
%
%% The first step (Line 2) divides the nodes of the training set across all the batches. The nodes within each batch represent the {\em root} nodes for the next step.
%% %
%% The second step (Line 4) constructs a sub-graph for every batch by sampling a subset of the root nodes' neighborhood.
%
In this section, we propose community-aware randomization schemes for the two steps of mini-batch construction (Algorithm~\ref{alg:minibatch}) that allows combining the convergence benefits of randomization with the data reuse benefits of structure-awareness.
%
Our proposal requires the community membership of nodes in the graph which is available to us once we perform community-based graph reordering\footnote{While we use a reordering mechanism based on hierarchical community detection via modularity maximization~\cite{rabbit}, \sysname can work with any community detection algorithm and also does not strictly require the graph to be community-ordered.}.
%%

%% \subsection{Knobs for biased mini-batch construction}
%% \begin{itemize}
%%     \item Using a diagram or the algorithm, highlight the two knobs/steps in mini-batch creation: (a) selecting the root nodes and (b) selecting the (sampled) neighbors of the root nodes
%%     \item Re-iterate that the current de-facto standard is to use {\em uniform} randomization for both knobs
%%     \haggai{I suggest to have an illustration showing both knobs.} \VB {Agreed! will work on a variation of the diagram we used in our NTECH submission}
%% \end{itemize}

\subsection{Biased partitioning of root nodes to batches} \label{subsec:bias-root-partitioning}
The baseline mini-batching approach randomly and uniformly distributes the nodes of the training set across mini-batches.
%
Specifically, during each training epoch, the contents of the training set are shuffled in a uniform random manner and then the elements of the shuffled set are mapped to batches as demonstrated in the top left panel of Figure~\ref{fig:biased-root-selection}. 
%
With uniform randomization, the root nodes within each mini-batch often belong to different communities which is sub-optimal for data reuse (as discussed in the previous Section~\ref{sec:rand-vs-structure}, the cache locality benefits of reordering primarily comes from processing members of a community together).
%
In contrast, the top-right panel of Figure~\ref{fig:biased-root-selection} shows the effect of not randomizing the training set before mapping the root nodes to batches.
%
In this case, the root nodes within batches are all mostly from the same community and the partitioning of root nodes to batches is static across all training epochs.
%
While great for data reuse and per-epoch runtime, such a scheme would suffer from poor convergence (Figure~\ref{fig:rand-vs-norand-extreme}).
%%

\begin{figure}[t]
    \centering
    \includegraphics[keepaspectratio,width=0.9\columnwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Figures/root-node-randomization.pdf}
\caption{{\bf Biased Root Partitioning:} 
{\em Communities in the training set are shown with different colors. For the sake of simplicity, we do not show community-wide randomization for the community-aware schemes in the bottom row. In practice, communities are also shuffled as whole blocks in addition to randomizing the contents within community boundaries.}
}
%\vspace{-4ex}
\label{fig:biased-root-selection}
\end{figure}


Aiming to find a good balance between randomization and community awareness in the root node partitioning step, we propose {\em community-aware} randomization of the training set before mapping root nodes to mini-batches (the star under Line-2 of Algorithm~\ref{alg:minibatch} identifies the step we modify).
%
Specifically, within the training set, we treat each community as a block and then apply two levels of randomization: (1) We shuffle the communities around as whole blocks, and (2) we also shuffle the contents within each community block.
%
As illustrated in the bottom-left panel of Figure~\ref{fig:biased-root-selection}, this constrained form of randomization results in the root nodes of each mini-batch to mostly belong to the same community (similar to the no randomization policy) while also ensuring that the root nodes of each batch are shuffled every epoch (similar to uniform randomization).
%%

To allow users to vary the level of community structure-bias and randomness during mini-batch creation, we add a knob to the scheme described in the previous paragraph.
%
Instead of restricting randomization at the granularity of a single community, we allow a fixed number of communities to be {\em mixed} to form a super-community and then restrict randomization to within the super-community boundary. 
%
Increasing the number of communities that are mixed, increases the amount of randomization and reduces the community-bias during mini-batching and vice versa.
%
The bottom-right panel of Figure~\ref{fig:biased-root-selection} shows the effect of mixing two communities which creates mini-batches that fall in between the batches of uniform randomization and no randomization.
%
In order to perform community-aware biased root selection as depicted in the bottom row of Figure~\ref{fig:biased-root-selection}, we only require the community information of each node in the graph which is available to us after performing community-based reordering.
%
{\bf In summary, the \sysname knob for controlling the community structure bias in partitioning root nodes is the number of communities to mix before randomization (value ranges from 0 to number of communities in the training set).}
%%

%% \haggai{consider explicitly specifying the knobs that we end up with - what is the input to the algorithm.}

\subsection{Biased neighborhood sampling} \label{subsec:biased-ngh-sampling}
Once the root nodes of each mini-batch are known, the next step is to traverse the $L$-hop neighborhood of the root nodes (for a $L$-layer GNN) and sample a subset of the neighbors to form the sub-graph associated with each batch (star under Line-4 of Algorithm~\ref{alg:minibatch}).
%
Figure~\ref{fig:biased-ngh-selection} shows the sub-graph created for a two-layer GNN operating on the example reordered graph from Figure~\ref{fig:reordering-example}.
%
The baseline approach samples these neighbors in a uniform random manner where each neighboring node has an equal likelihood of being selected.
%
Consequently, the sub-graph with uniform random neighbor sampling consists of nodes spanning multiple communities which increases the batch's data footprint and increases the cache pressure.
%
A community-biased sampling approach differentiates between {\em intra-} and {\em inter-}community edges and samples neighbors belonging to the same community with a higher probability.
%
The right-panel of Figure~\ref{fig:biased-ngh-selection} illustrates that prioritizing intra-community edges results in a smaller sub-graph for the same root nodes.
%
We set the probability of sampling intra-community edges as $p$ and inter-community edges as $1-p$.
%
{\bf The \sysname knob for controlling the community structure bias during neighborhood sampling is $p$ where values range from 0.5 (equal likelihood of selecting all neighbors) to 1.0 (only select neighbors from the same community).}
%%

\begin{figure}[t]
    \centering
    \includegraphics[keepaspectratio,width=0.9\columnwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Figures/biased-ngh-selection.pdf}
\caption{{\bf Biased Neighborhood Selection:} 
{\em Biased neighborhood selection for the graph in Figure~\ref{fig:reordering-example}. Intra-community edges are highlighted with blue and inter-community edges are highlighted with red. For a 2-layer GNN, uniform random neighborhood sampling creates a larger sub-graph compared to a biased scheme where intra-community neighbors are selected with a higher probability.}
}
%\vspace{-3ex}
\label{fig:biased-ngh-selection}
\end{figure}

%{\bf Interaction between the two biased steps: }
%
In this section, we proposed community-aware randomization schemes for both root node partitioning and neighborhood sampling.
%
Additionally, we exposed knobs to control the level of community structure bias in the two steps.
%
In Section~\ref{sec:eval}, we will evaluate GNN training across different combinations of knobs for biased root partitioning and biased neighborhood sampling and demonstrate how controlling the level of graph structure bias yields different points on the per-epoch runtime vs convergence trade-off space.
%%

%% \haggai{I suggest to add another algorithm box here with our two new knobs}

%% \begin{itemize}
%%     \item \VB{Maybe mention that this approach could be extended a few different ways -- we could assign a different score for each edge (i.e. treat intra-community edges of different communities differently) or we could even leverage entirely different graph structural properties (such as hubs in power-law graphs and is not just restricted to community structure)}
%%     \item \VB{TODO: Run experiments to see if other graph structural properties, besides community detection, can offer superior performance with biased mini-batch construction? Furthermore, is there a "best" graph structural property to leverage for each graph or can community-structure be a catch-all for all real-world inputs}
%%     \item \haggai{we should specify formally the different approaches that we propose. }
%% \end{itemize}




==> conclusions.tex <==
%\section{Conclusions} \label{sec:conclusions}
%
%In this work, we highlight the tension in mini-batch construction between the need for randomization (for good accuracy and convergence) and the need to be aware of the graph's structure (for good per-epoch performance).
%
%We show that \sysname offers a way out of this dichotomy and allows practitioners to find the right balance between graph structural bias and randomization during mini-batching to improve overall training performance.
%%

\section{Conclusions} \label{sec:conclusions}
%
In this work, we highlight the tension in mini-batch construction between the need for randomization (for good accuracy and convergence) and the need to leverage the graph's community structure (for efficient per-epoch processing). We demonstrate that \sysname resolves this dilemma by introducing controllable structure-aware randomization that balances these competing requirements. By providing knobs that adjust the degree of community bias during mini-batching, \sysname enables practitioners to optimize the trade-off between convergence rate and computational efficiency, achieving up to 2.76$\times$ (1.8$\times$ on average) faster training while maintaining accuracy within 1.79\% points (0.42\% on average) of traditional approaches.

==> evaluation.tex <==
\section{Evaluation} \label{sec:eval}

We perform an extensive analysis of the impact of \sysname based mini-batching on GNN training by sweeping different combinations of the knobs presented in Section~\ref{sec:biased-rand}.
%
Specifically, we characterize how changing the level of graph structure bias affects various training metrics   .
% 
We also compare \sysname against prior work on mini-batch construction for GNNs and measure \sysname's sensitivity to software caches for reducing CPU-GPU communication, L2 cache capacity, and hyper-parameter tuning.
%
%% Finally, we measure the sensitivity of \sysname across different GNN models, hyper-parameters, and GPUs.
%%

\subsection{Quantitative analysis of biased mini-batching} \label{subsec:main-knob-sweep}

We evaluate the effectiveness of different levels of community biased mini-batching on four training metrics -- final validation accuracy, per-epoch training time, number of epochs until convergence, and total training time.
%
The rows of Figure~\ref{fig:metrics-vs-knobs} correspond to each of the above metrics and the columns of the figure show results across different graphs.
%
Within each subplot, the different bars/colors represent different root node partitioning schemes (Table~\ref{table:root-mapping-policies}) and the x-axis represents different values of the intra-community probability knob from Section~\ref{subsec:biased-ngh-sampling}.
%
In Figure~\ref{fig:metrics-vs-knobs}, the setting ({\tt RAND-ROOTS} \& $p=0.5$) represents uniform random mini-batching baseline and ({\tt NORAND-ROOTS} \& $p=1.0$) represents the entirely community-based mini-batching scheme from Section~\ref{sec:rand-vs-structure}.
%
Other combinations of root node partitioning schemes and $p$ values represent \sysname with varying levels of community bias during mini-batching.
%% 

%\haggai{perhaps add "main baseline" or similar in the figure?}

%\haggai{not clear what the 50 percent stands for? is it the probability of the sampling inside the community?  this would be weird since uniform sampling for in the baselines lie GRAPHSAGE means that take all neighbors and sample uniformly from them without any knowledge of the clustering. need to clarify}.

%\haggai{ we need to explicitly writen the baseline names, eg COMM-RAND MIX XXX \% and explain what each baseline means. I suggest to add a paragraph about that in the previous section}
%%

We make two broad observations across the results in Figure~\ref{fig:metrics-vs-knobs}.
%
First, while the level of graph structure bias affects the final accuracy, the validation accuracy is always within 1.79\% point of the baseline (with the exception of entirely community-based mini-batching for {\tt ogbn-papers100M} which incurs a 4\% point accuracy loss likely due to its shorter maximum epoch limit). 
%
Second, we often observe a trade-off between per-epoch training speedup and the number of epochs until convergence.
%
Over the next few subsections, we will characterize how different levels of community structure bias in \sysname mini-batching impact the per-epoch time and convergence (in turn, affecting the overall speedup).
%%

\begin{figure*}[h!]
    \centering
    \includegraphics[keepaspectratio,width=1.0\textwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/allmetrics-vs-biased-knobs_gpu-a100-sxm4-80gb.pdf}
    \caption{{\bf Impact of \sysname across different GNN training metrics (rows) and input graphs (columns):}
    {\em All results (besides accuracy) are normalized to the baseline ({\tt RAND-ROOTS} \& $p=0.5$). The y-axis for val. acc. does not start from 0. } 
    }
    %\vspace{-2.5ex}
    \label{fig:metrics-vs-knobs}
\end{figure*} 
%
%\gal{This figure is overloaded, and it is hard to figure out what the message is. IT seems it is trying to do two things at the same time: Compare our COMM-RAND with baselines, and also show robustness to the HP. Can we separate into to different figures? Do we really need three values of p for all those cases?  It would be much mire clear if we pick a few representative experiments and show them at a decent size, then put the rest in a supplemental/ appendix.  Also, we should change the color scheme: Make all COMM_Rand different shadows of green, moving from light to dark and the parameters changes from $0\%$ to $50\%$}

%% \begin{figure*}[h!]
%%     \centering
%%     \includegraphics[trim=850 0 0 0 , clip,keepaspectratio,width=0.8\textwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/allmetrics-vs-biased-knobs_gpu-a100-sxm4-80gb.pdf}
%%     \caption{{\bf Impact of biased mini-batch construction on GNN training accuracy, convergence, and runtime} \haggai{this is currently not readable. We need to either split this into several plots or put it horizontally on the same page but much larger} \VB{I will increase the font sizes for this plot but does it maybe make sense to split this plot into 4 separate rows?} \haggai{perhaps add a title above each row specifying the metric?} \gal{avoid repeating the same legend. }
%%     }
%%     \label{fig:metrics-vs-knobs}
%% \end{figure*} 
%% 
%% 
%% \begin{figure*}[h!]
%%     \centering
%%     
%%     \includegraphics[trim=0 0 850 0 , clip,keepaspectratio,width=0.8\textwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/allmetrics-vs-biased-knobs_gpu-a100-sxm4-80gb.pdf}
%%     \caption{{\bf Impact of biased mini-batch construction on GNN training accuracy, convergence, and runtime} \haggai{this is currently not readable. We need to either split this into several plots or put it horizontally on the same page but much larger} \VB{I will increase the font sizes for this plot but does it maybe make sense to split this plot into 4 separate rows?} \haggai{perhaps add a title above each row specifying the metric?} \gal{avoid repeating the same legend. }
%%     }
%%     \label{fig:metrics-vs-knobs}
%% \end{figure*} 

%\haggai{general comment - we need to add more numbers. when we say that something archives speedup, lets try to say by how much}

\subsubsection{Impact on Per-Epoch Training Time} \label{subsec:per-epoch-explanation}
The second row in Figure~\ref{fig:metrics-vs-knobs} reports per-epoch training speedups relative to the baseline of uniform random mini-batching ({\tt RAND-ROOTS} \& $p=0.5$).
%

\textbf{The impact of root node partitioning:} We first discuss the impact of different root node partitioning policies on per-epoch times (and focus on the results with no intra-community bias during neighborhood sampling $p=0.5$).
%
As mentioned in Section~\ref{sec:methodology}, we use community-reordered inputs for all our evaluations.
%
Therefore, the highest per-epoch speedups are achieved when no randomization is performed before partitioning the root nodes across batches ({\tt NORAND-ROOTS}) because the graph's ordering is optimized for high data reuse from caches (Section~\ref{subsec:graph-reordering}).
%
On average, ({\tt NORAND-ROOTS} \& $p=0.5$) offers 1.69x per-epoch speedups over the baseline.
%
Community-aware randomization without any community mixing ({\tt COMM-RAND-MIX-0\%}) often achieves the next best per-epoch speedups (1.32x on average) because it creates mini-batches with root nodes that mostly belong to the same community but deviates slightly from the reuse-optimized ordering. 
%
%\VB{Maybe also mention the loss of hierarchical community structure -- our schemes only track outermost community boundaries}.
%
Once we start mixing communities ({\tt COMM-RAND-MIX-\{12.5\%,25\%,50\%\}}), we see a further reduction in per-epoch speedups (with speedups decreasing as more communities are mixed).
%
Even with the \sysname version with the least amount of community structure bias ({\tt COMM-RAND-MIX-50\%}), we notice an average per-epoch speedups of 1.09x over the baseline because the memory access pattern still has a small level of community bias that improves data reuse in caches.

\textbf{The impact of intra-community bias during neighborhood sampling ($p$):} 
%
Increasing $p$ has a straightforward impact on per-epoch performance -- as the likelihood of selecting intra-community edges increases, the per-epoch speedup also increases because the sub-graphs associated with batches are more aligned with the community structure of the graph.
%
Furthermore, increasing the intra-community bias during neighbor selection tends to improve per-epoch speedups across {\em all} root node partitioning policies.
%%

\begin{figure}[ht]
    \centering    \includegraphics[keepaspectratio,width=\columnwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/per-epoch-time-vs-featsize_mean.pdf}
    \caption{{\bf Per-epoch training time vs input node features size:} 
    {\em Different points of the same color represent different levels of community bias during neighborhood sampling ($p$) for the same root node partitioning policy. The titles also report the pearson correlation between per-epoch time and input feature size for each graph. } 
    }
    %\vspace{-3ex}
    \label{fig:perepochtime-vs-featsize}
\end{figure}
%\gal{Increse font size on axes and legend. Change the color scheme like I suggested above: all COMM_RAnd in different shades of green.}

\textbf{Discussion:} Results indicate that \sysname mini-batching primarily improves per-epoch training time by reducing the size of the sub-graphs per batch which reduces the footprint of the input feature data that needs to be fetched for the training computations.
%
To corroborate this, Figure~\ref{fig:perepochtime-vs-featsize} shows the correlation between per-epoch time and the average size of the input feature data ($X$) corresponding to the nodes within batches.
%
Across root node partitioning policies, we see that the average input node features size decreases as the level of community-bias increases from {\tt RAND-ROOTS} to {\tt COMM-RAND-MIX-50/25/12.5\%} to {\tt COMM-RAND-MIX-0\%} to {\tt NORAND-ROOTS} root node partitioning policies.
%
Within the same root node partitioning policy, we also see that increasing levels of intra-community bias during neighbor sampling (higher $p$) also reduces the input feature size.
%
The smaller input feature sizes across batches translate to higher data reuse in software and on-chip caches as demonstrated in Sections~\ref{subsubsec:sw-gpu-cache} and ~\ref{subsec:l2-cache-sensitivity} respectively.
%%

%\christos{also give reader an intuition about when to stop optimizing/turning knobs. When do you reach diminishing return in performance anyway due to X and Y hardware characteristics.} \VB{We could emphasize this point by linking per-epoch speedups to the level of input feature footprint reduction?}

\subsubsection{Impact on convergence}
The third row in Figure~\ref{fig:metrics-vs-knobs} shows the increase in number of epochs until convergence relative to the baseline (lower values are desirable).
%
In the previous subsection, we noticed that as the level of community-bias in \sysname mini-batching increased, the per-epoch speedups also improved. 
%
%(with the highest per-epoch speedups corresponding to completely community-based mini-batching ({\tt NORAND-ROOTS} \& $p=1.0$).
%
We observe nearly the opposite trend for convergence -- higher levels of community-bias in \sysname lead to greater delays in convergence.
%completely community-based mini-batching incurs the highest delays in convergence compared to the baseline (requiring 1.6x more epochs on average).
%
For biased neighborhood sampling with $p=1.0$, the average increase in the number of epochs until convergence (relative to uniform random baseline) is 1.23x, 0.99x, 1.01x, and 0.85x with {\tt COMM-RAND-MIX-0\%}, {\tt COMM-RAND-MIX-12.5\%}, {\tt COMM-RAND-MIX-25\%}, and {\tt COMM-RAND-MIX-50\%} respectively. 
%%
%% Among community-aware randomization schemes, mixing more communities often helps with convergence.
%% %
%% \VB{Dont have a good explanation for two trends -- (1) we sometimes see better convergence with more intra-community bias during neighbor selection and (2) it is unclear how we sometimes *improve* convergence over the baseline?}
%%

\begin{figure}[ht]
    \centering    \includegraphics[keepaspectratio,width=\columnwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/epochs-vs-numlabels_mean.pdf}
    \caption{{\bf No. of epochs to converge vs label diversity:} 
    {\em A higher average no. of labels per batch is correlated to faster convergence. Note that the labels are only associated with root nodes and, therefore, different levels of community bias in neighborhood sampling ($p$) has no impact on the label count}
    }
    %\vspace{-2.5ex}
    \label{fig:epochs-vs-numlabels}
\end{figure}

%% Analyzing the impact of biased mini-batching on convergence is complicated by \haggai{due to?} the use of learning rate scheduling. 
%% %
%% While essential for ensuring comparable accuarcy to the baseline, the learning rate scheduler accounts for the difference in gradient update across different mini-batching schemes and changes training dynamics accordingly.
%
Prior work~\cite{chiang2019cluster} observed that the convergence of GNN training is improved when the label entropy among batches is high.
%
Figure~\ref{fig:epochs-vs-numlabels} reports the relationship between number of epochs until convergence and the average number of labels per batch.
%
While the correlations are not as strong as Figure~\ref{fig:perepochtime-vs-featsize}, a higher label diversity within batches is correlated with lower number of epochs until convergence.
%
The result shows that as the level of community bias increases (from {\tt RAND-ROOTS} to {\tt NORAND-ROOTS}), the average number of labels per batch decreases which leads to delayed convergence.
%%

\subsubsection{Best \sysname knobs}

The previous subsections showed a trade-off between per-epoch training time and the number of epochs until convergence.
%
As the level of community-bias in \sysname mini-batching increases, we see higher per-epoch speedups and greater delay in convergence and vice versa.
%
Total training time is a product of per-epoch time and the number of epochs. 
%
Therefore, the last row of Figure~\ref{fig:metrics-vs-knobs} has less obvious trends across different root node partitioning policies and intra-community probabilities ($p$).
%
However, our evaluation shows that root node partition schemes with community mixing combined with maximum intra-community bias during neighbor sampling ($p=1.0$) provides a good balance between per-epoch speedup and convergence.
%
Across all datasets, we find that {\tt COMM-RAND-MIX-12.5\%} $+$ $p=1.0$ provides the higher average total training speedups of 1.8x (with speedups ranging from 1.14x to 2.76x).
%
Selecting other root node partitioning policies does not result in a major performance cliff -- {\tt \seqsplit{COMM-RAND-MIX-25\%}} leads to an average net speedup of 1.6x (range from 1.16x to 2.05x) and {\tt COMM-RAND-MIX-50\%} leads to an average net speedup of 1.62x (range from 1.21x to 2.03x).
%%

The above discussion on the best \sysname knob configuration assumed a scenario where the GNN is trained until convergence.
%
If instead, the GNN is trained for a fixed number of epochs, then a higher level of community-bias in \sysname mini-batching would be more desirable.
%
Finally, we note that the knobs exposed in Section~\ref{sec:biased-rand} can allow users to find the right level of community bias for their unique combinations of dataset, GNN model, and GPU architecture. It may even be possible to cast the problem of finding the right bias level as a learning problem in itself and we leave this exploration for future work. 
%%\haggai{nice}
%%

\subsection{Impact of hyperparameter tuning} \label{subsec:hyperparam-tuning}

The results so far were collected using the default hyper-parameters from the DGL reference implementations.
%
\sysname introduces two new hyper-parameters -- root node partitioning policy and community bias during neighborhood sampling (as described in Section~\ref{sec:biased-rand}).
%
A natural question is whether the additional cost of hyperparameter tuning with two extra parameters would overshadow \sysname's benefits showcased in the previous section.
%
To answer this question, we performed an experiment with fixed budgets for hyperparameter tuning and training using the {\tt reddit} dataset.
%
For both the baseline and \sysname, we perform a random search for 1 hour (we sweep the 5 hyper-parameters mentioned in Section~\ref{sec:methodology} for the baseline and 7 hyper-parameters for \sysname).
%
Due to its higher performance, \sysname explores 70 hyper-parameter combinations compared to 62 combinations with the baseline.
%
Next we trained both the baseline and \sysname versions with the best hyper-parameters for 30 minutes and Table~\ref{table:hyperparam-sweep} reports the results.
%
Due to superior per-epoch performance, \sysname is able to train for 1.54x more epochs compared to the baseline within the same training budget.
%
Consequently, \sysname trains a model which achieves a higher final validation accuracy and also improves the inference accuracy by 0.27\% points.
%
This result demonstrates that \sysname is able to offer benefits even after accounting for the hyperparameter tuning costs.
%%

\begin{table}[ht]
    \caption{{\bf \sysname's effectiveness after hyperparameter tuning:}
    {\em Results after training for 30 minutes (using the best hyper-parameters). \sysname trains for more epochs leading to improved model accuracy}
    }
    \label{table:hyperparam-sweep}
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccc}
    \hline
                       & \multicolumn{1}{l}{\textbf{No. of Epochs}} & \multicolumn{1}{l}{\textbf{Final Val. Acc}} & \multicolumn{1}{l}{\textbf{Test Acc}} \\ \hline
    \textbf{Baseline}  & 641.8                                      & 96.10\%                                     & 96.30\%                               \\ 
    \textbf{COMM-RAND} & 987.6                                      & 96.22\%                                     & 96.57\%                               \\ \hline
    \end{tabular}%
    }
\end{table}


\subsection{Comparison to prior work on mini-batching} \label{subsec:prior-work-comparison}

{\bf Structure-agnostic randomized mini-batching: }
%
As discussed in Section~\ref{sec:background}, most prior-work on mini-batch construction ignores the graph structure.
%
We choose LABOR as a representative among this class of mini-batching policies because it was shown to outperform LADIES~\cite{labor} (which, in turn, outperforms FastGCN~\cite{ladies}).
%
After 25 epochs of training on the {\tt reddit} dataset, LABOR achieved an accuracy of 96.08\% (compared to 96.21\% with the uniform random mini-batching baseline) while improving the per-epoch processing time by 1.1x compared to the baseline.
%
In comparison, \sysname achieves an accuracy of 95.25\% while providing a higher per-epoch speedup of 1.75x.
%
LABOR (and other related mini-batching schemes) do not take into account the community structure of graphs and, therefore, miss out on the opportunity to significantly improve data reuse.
%%

%% \begin{table}[ht]
%% \caption{{\bf Comparing structure-agnostic mini-batching schemes}}
%% \label{table:structure-agnostic-minibatching}
%% \centering
%% \resizebox{\columnwidth}{!}{%
%% \begin{tabular}{|l|c|c|c|c|}
%% \hline
%%  & {\bf Baseline} & {\bf Comm-Rand} & {\bf LABOR} & {\bf LADIES}  \\
%% \hline
%% {\bf Final Val. Acc (\%)} & 96.13 & 95.25 & 96.08 & \\
%% \hline
%% {\bf Per-Epoch Time (s)} & 5.28 & 2.99 & 5.04 & \\ 
%% \hline
%% \end{tabular}%
%% }
%% \end{table}

{\bf Structure-aware randomized mini-batching: }
%
ClusterGCN~\cite{chiang2019cluster} is the prior work most closely related to ours because they also combine randomization and graph structure while creating mini-batches.
%
Specifically, ClusterGCN uses METIS~\cite{metis} to partition the graph and then forms mini-batches by randomly combining a fixed number of graph partitions.
%
Both graph partitioning and community-detection (used by \sysname) find regions of high inter-connectivity within graphs but differ in the same way as k-means clustering differs from agglomerative clustering.
%
Graph partitioning requires the user to specify the number of partitions whereas community-detection determines the appropriate number of communities based on the graph structure.
%
However, the differences between ClusterGCN and our work (\sysname) run deeper than the choice of using graph partitioning versus community-based reordering.
%%

\begin{table}[ht]
\caption{{\bf Comparison against clusterGCN across datasets}:
{\em Results after 25 epochs of training}
}
\label{table:clustergcn-comparison}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\hline
              & \multicolumn{2}{c}{\textbf{Baseline}}                                 & \multicolumn{2}{c}{\textbf{COMM-RAND}}                                & \multicolumn{2}{c}{\textbf{ClusterGCN}}                               \\ 
              \midrule 
              & \multicolumn{1}{l}{Per-Epoch } 
              & \multicolumn{1}{l}{Val.  \%} & \multicolumn{1}{l}{Per-Epoch } & \multicolumn{1}{l}{Val. \%} & \multicolumn{1}{l}{Per-Epoch } & \multicolumn{1}{l}{Val. \%} \\ 
              & \multicolumn{1}{l}{ Speedup} 
              & \multicolumn{1}{l}{ Acc \%} 
              & \multicolumn{1}{l}{  Speedup} & \multicolumn{1}{l}{Acc \%} 
              & \multicolumn{1}{l}{  Speedup} & \multicolumn{1}{l}{Acc \%} \\ 
              
              \midrule 
              
reddit        & \multicolumn{1}{c}{1.0x}      & 96.13                            & \multicolumn{1}{c}{1.76x}           & 95.25                            & \multicolumn{1}{c}{2.10x}           & 93.45                            \\ 
igb-small     & \multicolumn{1}{c}{1.0x}          & 74.77                            & \multicolumn{1}{c}{1.68x}          & 74.64                            & \multicolumn{1}{c}{5.94x}              & 74.58                            \\ 
ogbn-products & \multicolumn{1}{c}{1.0x}           & 91.02                            & \multicolumn{1}{c}{2.04x}           & 89.87                            & \multicolumn{1}{c}{0.26x}          & 89.4                             \\ 
ogbn-papers100M   & \multicolumn{1}{c}{1.0x}          & 63.29                            & \multicolumn{1}{c}{1.48x}          & 62.15                            & \multicolumn{1}{c}{0.08x}         & 50.78                            \\ \bottomrule
\end{tabular}%
}
%\vspace{-3ex}
\end{table}

There are two fundamental differences between ClusterGCN and our proposal of \sysname mini-batching.
%
First, ClusterGCN performs a more limited form of randomization compared to our proposal.
%
While ClusterGCN creates mini-batches by randomly combining different graph partitions, the contents within each partition are not randomized.
%
In contrast, our community-aware randomization schemes shuffle entire communities as well as randomizing the contents within each community (Figure~\ref{fig:biased-root-selection}).
%
Consequently, ClusterGCN converges more slowly in comparison to our proposal and consistently achieves lower accuracy compared to \sysname (Table~\ref{table:clustergcn-comparison}).
%
Second, ClusterGCN creates mini-batches by composing entire graph partitions and does not take the training set into account during mini-batch construction.
%
Therefore, ClusterGCN is required to evaluate the {\em entire} graph during training.
%
For graphs with large training sets ({\tt reddit} \& {\tt igb-small} have 65\% and 60\% of the graph's nodes labeled respectively), ClusterGCN is effective at improving per-epoch time over the baseline (Table~\ref{table:clustergcn-comparison}).
%
However, when the training set is small ({\tt ogbn-products} and {\tt ogbn-papers100M} have only 20\% and 1\% of the graph's nodes labeled), ClusterGCN is significantly slower than the baseline (by up to 13x).
%
In contrast, \sysname offers consistent speedups because we only perform computations on the subset of the graph connected to the nodes in the training set.
%
Figure~\ref{fig:perepoch-vs-trainidx-sweep} further illustrates this inefficiency of ClusterGCN.
%
When the training set size of {\tt reddit} is artificially reduced, we observe that the per-epoch training time with ClusterGCN remains constant while both the baseline and \sysname mini-batching offer lower per-epoch processing times as the training set size shrinks.
%
Therefore, ClusterGCN is unlikely to be effective in the more realistic GNN training scenario where only a small percentage of the graph's nodes are labeled.
%%

\begin{figure}[ht]
\centering
\includegraphics[keepaspectratio,width=0.9\columnwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/per-epoch-time_vs_trainidxsweep_gpu-ada-rtx-6000.pdf}
\caption{{\bf Per-Epoch time vs training set size:}
{\em ClusterGCN performance is invariant to the training set size}
%in contrast to the runtime with baseline and \sysname mini-batching}
}
%\vspace{-2.5ex}
\label{fig:perepoch-vs-trainidx-sweep}
\end{figure}

\subsection{Generalizing to other GNN models} \label{subsec:other-gnn-models}

The results up to this point have focused on the GraphSAGE model. 
%
However, \sysname generalizes to arbitrary GNN models.
%
To illustrate this point, we performed a sweep of different \sysname knobs (as performed in Figure~\ref{fig:metrics-vs-knobs}) on two other popular GNN models -- Graph Convolution Network (GCN)~\cite{kipf2016semi} and Graph Attention Network (GAT)~\cite{velivckovic2017graph}.
%
Table~\ref{table:other-gnn-models} shows different training metrics for the {\tt reddit} dataset where the baseline is {\tt RAND-ROOTS} $+$ $p = 0.5$ and \sysname reports results for the knobs that achieve the best balance between accuracy and performance.
%
The results show that for both the GCN and GAT, \sysname achieves a final validation accuracy that is within 1\% points of the baseline while improving both the per-epoch and total training times.
%
\sysname achieves a total training speedup of 2.03x and 1.38x for GCN and GAT respectively.
%%

%
%% GCN and GraphSAGE perform simple computations on neighbors' embeddings (summation and mean calculation respectively) and, therefore, are limited by data movement of node feature data.
%% %
%% Since \sysname is a data-reuse optimization, it is equally effective across GCN and GraphSAGE.
%% %
%% In contrast, GAT is more computationally-intensive and community-biased mini-batching offers lower speedups for GAT.
%% %%

%% \begin{figure}[ht]
%% \centering
%% \includegraphics[keepaspectratio,width=\columnwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/cross-gnn-network-speedups.pdf}
%% \caption{{\bf Per-Epoch Speedups across GNN models} 
%% }
%% %\vspace{-1.0ex}
%% \label{fig:cross-gnn-speedups}
%% \end{figure}

\begin{table}[ht]
    %\vspace{-3ex}
    \caption{{\bf \sysname's effectiveness for other GNN models:}
    {\em Results for the {\tt reddit} dataset.}
    }
    \label{table:other-gnn-models}
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{llcccc}
    \toprule
    &   & \multicolumn{1}{c}{Final Val.} & \multicolumn{1}{c}{Per-Epoch} & \multicolumn{1}{c}{ Num} & \multicolumn{1}{c}{Total Training } \\ 
    &   & \multicolumn{1}{c}{Acc. \%} & \multicolumn{1}{c}{Time (s)} & \multicolumn{1}{l}{Epochs} & \multicolumn{1}{c}{Time (s)} \\ 
    \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} {\bf GCN} \end{tabular}}   & Baseline  & 78.67 & 3.42   & 50.4   & 172.18    \\  
    \cline{2-6} 
    & COMM-RAND & 77.82   & 2.86    & 29.6   & 84.56   \\ \midrule
    \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} {\bf GAT} \end{tabular}} & Baseline  & 90.60                                  & 2.00                                    & 51.0                               & 102.05                                       \\ \cline{2-6} 
         & COMM-RAND & 90.09                                  & 1.74                                    & 42.4                               & 73.72                                       \\ \bottomrule
    \end{tabular}%
    }
    \vspace{-1.5ex}
\end{table}

%%\subsection{Sensitivity studies \textcolor{red}{[NEW]}} \label{subsec:sensitivities}

\subsection{Sensitivity studies}
\subsubsection{Impact of software-managed caches.} \label{subsubsec:sw-gpu-cache}
%
As mentioned in Section~\ref{sec:methodology}, due to the large size of the {\tt \seqsplit{ogbn-papers100M}} dataset we could not fit the graph and features all on the GPU memory and, therefore, we performed mixed CPU$+$GPU training for this dataset.
%
Specifically, the graph and feature data are stored on the CPU memory while the model is on the GPU memory.
%
During neighborhood sampling, the relevant parts of the graph and feature data are moved from the CPU to the GPU using Unified Virtual Addressing (UVA)~\cite{uva, dgl-dataloader-api}.
%
The DGL framework provides an API for a software-managed cache that is resident in the GPU memory and allows reuse in feature accesses to reduce the amount of UVA transfers.
%
Figure~\ref{fig:sw-gpu-cache} compares the per-epoch speedups achieved with \sysname without any software caching (the results in Figure~\ref{fig:metrics-vs-knobs}) with per-epoch speedups in the presence of a software cache capable of storing 4M node features.
%
The result shows that the presence of a software cache allows \sysname to provide higher per-epoch training speedups.
%
The more community-biased versions of \sysname (i.e. {\tt \seqsplit{COMM-RAND-MIX-\{12.5\%,0\%\}}} $+$ $p=1.0$) offer greater speedups due to their ability to achieve higher reuse in the software cache.
%
With the software cache, the uniform random baseline experiences a miss rate of 35.46\% whereas the different \sysname versions from {\tt COMM-RAND-MIX-50\%} to {\tt COMM-RAND-MIX-0\%} experience miss rates of 20.99\%, 11.39\%, 6.22\%, and 6.21\% respectively.
%
Lastly, the software cache used in this experiment employs the LRU replacement policy~\cite{merlin-gpu-cache}.
%
Extending the software cache to use more graph-centric cache replacement policies~\cite{popt-hpca21,grasp-hpca20} could further boost \sysname's performance improvements and we will explore \sysname's effectiveness in caching node feature data~\cite{bgl-nsdi23,pagraph-socc20,global-neighborhood-sampling} as part of future work.
%%

\begin{figure}[h]
\centering
\includegraphics[keepaspectratio,width=1.0\columnwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/sw-gpu-cache-perepoch-speedups.pdf}
\caption{{\bf Per-Epoch Training Speedups with a SW cache:}
{\em \sysname increases performance by reducing UVA transfers between CPU and GPU (for {\tt ogbn-papers100M}).}
}
%\vspace{-1.5ex}
\label{fig:sw-gpu-cache}
\end{figure}


\subsubsection{Sensitivity to on-chip cache capacity} \label{subsec:l2-cache-sensitivity}

The main reason for per-epoch training speedups with \sysname is due to reducing the working set size and improving on-chip cache reuse (Figure~\ref{fig:perepochtime-vs-featsize}).
%
To further explore \sysname's effectiveness a function of the L2 cache capacity, we used Multi-Instance GPU (MIG)~\cite{mig} to create GPU partitions with reduced L2 cache capacities.
%
An A100 GPU features a 40MB L2 cache and with MIG we created GPU partitions with 1/2 and 1/4 the number of SMs and memory capacity which have 20MB and 10MB L2 caches respectively.
%
Figure~\ref{fig:l2-cache-sensitivity} shows the per-epoch speedups with different \sysname configurations (with $p=1.0$) for the {\tt reddit} dataset across different L2 cache capacities.
%
The results show that as the L2 cache size decreases (or the ratio of the working set size relative to the cache capacity increases), we see higher per-epoch speedups across the different \sysname configurations.
%
While using MIG partitions is not a perfect experiment for a cache sensitivity study (because MIG also cuts the number of SMs and available memory bandwidth along with the L2 cache capacity), these results provide an estimate of \sysname's continued effectiveness as the ratio of the problem size relative to the cache capacity increases.
%%

\begin{figure}[ht]
\centering
\includegraphics[keepaspectratio,width=\columnwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/mig-cache-sensitivity.pdf}
\caption{{\bf Per-Epoch Speedups vs L2 cache capacity:}
{\em Results normalized to the baseline for each L2 configuration.}
}
%\vspace{-1.5ex}
\label{fig:l2-cache-sensitivity}
\end{figure}

\subsubsection{Pre-processing overheads} \label{subsec:preprocessing-cost}
%
We assume that the graphs are already community-ordered for all runs (including the baseline) and, therefore, do not consider the pre-processing cost of reordering.
%
Furthermore, the overhead of graph reordering can be amortized over multiple epochs of GNN training (as well as inference).
%
Running RABBIT graph reordering on the {\tt reddit} dataset amounts to 0.78\% of the baseline's total training time.
%
Finally, \sysname only requires identifying the community membership of nodes and does not require the graph to be community-ordered which allows further reduction in pre-processing overheads.
%%

%% \subsection{Additional experiments}
%% \begin{itemize}
%%     \item How do we amortize reordering overheads? Do we really need the graph to be reordered or does we just need to distinguish between intra/inter-community edges?
%%     \item What is the impact of our idea when employed with hyperparameter tuning?
%%     \item What is the impact of final validation accuracy on stopping conditions? (Would different PATIENCE values, max epochs radically change the perf-vs-acc results?)
%%     \item How does our idea work with different GPUs? Identify trends with memory BW and cache capacity
%%     \item How does our idea work with different system settings? (Fully GPU vs mixed CPU-GPU vs mixed + GPU SW cache)
%%     \item \VB{Are there any ablation studies that would make sense here?}
%% \end{itemize}

==> intro.tex <==
\section{Introduction} \label{sec:intro}
%% \gal{Its not intuitive why the following simple sampling strategy would fail:  cover the graph by tightly connected components, and sample from those components. Lets convince the reader early that sampling is a hard problem} \haggai{this is one extreme point of our algorithm which is heavily biased towards structure. We show that randomness in both the root node selection and in neighbor sampling is critical. We mention that below, perhaps should move to the beginning? }
%% 
%% \gal{Suggested alternative: start with the problem, not with GNNs.}

Graphs are a primary type of data in many important applications ranging from social network analysis~\cite{gnn-socialrec} to financial fraud detection~\cite{gnn-frauddetection} with typical graphs containing millions of nodes and billions of edges. Graph neural networks (GNNs) have emerged as the primary tool for analyzing such graphs, but the scale of inputs poses significant computational challenges as the graph data far exceeds available memory capacity on GPUs. A common approach to addressing this limitation of GNN training is {\em mini-batching}, where the graph is divided into smaller chunks on which the model is then trained sequentially.

% \gal{See proposed alternative above}
% Graph Neural Networks (GNNs) have emerged as the primary tool for analyzing massive graphs. However, processing graphs with hundreds of millions of nodes and edges—such as social networks —poses significant computational challenges as these graphs far exceed available memory capacity. To address this limitation, mini-batching - a procedure in which the graph is effectively partitioned into several parts that are trained independently -  has become the predominant approach for training GNNs on large graphs.

GNN training via mini-batching faces two competing requirements. Randomization during training is essential for model accuracy and convergence \cite{bottou2009curiously, bengio2012practical, safran2020good, gurbuzbalaban2021random}, leading to widespread adoption of random sampling in GNN frameworks \cite{hamilton2017inductive, fey2019fast, wang2019deep}. However, graph analytics research has shown that exploiting graph structure through node reordering can significantly improve cache efficiency \cite{gorder,rabbit,cagra,when-is-reordering-opt,rabbitpp-ispass2023,grasp-hpca20,nested-dissection,parallel-rcm}. This is particularly effective for real-world graphs that exhibit community structure, where nodes are densely connected within communities but sparsely connected across communities. While this community-aware approach has proven effective for GNN inference \cite{grow-hpca23,gnnadvisor-osdi21}, its benefits are lost during training due to random sampling that harms locality.
The result is a clear trade-off: random mini-batching achieves good accuracy and convergence but with slow per-epoch computation, while structure-based mini-batching enables fast per-epoch computation but leads to slower convergence and reduced accuracy. This creates a significant performance dilemma for practitioners.
%%

%\haggai{Suggest adding something like:" Previous studies regarding efficient training of GNNs \cite{XXX} mostly overlooked this tension and failed to recognize and utilize the relationship between being structurally biased and randomization"}

%\haggai{consider stating from the start that our method is simple (in a good way) and effective. }
We present \sysname (Community-Structure-aware Randomized Mini-batching), a GNN training methodology to bridge this gap by introducing both structural bias and randomization into the mini-batching process in a controlled manner.
%
There are two main steps of mini-batch construction: (1) partitioning the nodes in the training set across batches and (2) building a sub-graph by sampling a subset of the neighborhood of nodes within each batch.
%
Conventional mini-batch construction uses uniform (or structure-agnostic) randomization for both steps which optimizes for fast convergence in a few epochs at the expense of slow per-epoch processing.
%
In contrast, we develop a constrained form of randomization that is aware of the community structure in graphs and use it to build mini-batches that are effective at improving per-epoch performance (due to community-bias) while also maintaining good convergence (due to randomization).
%
Furthermore, \sysname exposes knobs that allow controlling the level of structural-bias and randomness, enabling practitioners to explore the right balance between per-epoch processing and convergence rate to improve overall GNN training time.
%%
In summary, we make the following contributions in this paper:
%
\begin{itemize}
    \item We highlight the tension between randomization and graph structure awareness during GNN training by showing the pitfalls of both purely-random and purely-structure-based mini-batching approaches (\underline{Section~\ref{sec:rand-vs-structure}})
    \item We introduce {\em community structure-aware randomization} (\sysname) and provide knobs to balance the competing requirements of high per-epoch performance vs model convergence and accuracy (\underline{Section~\ref{sec:biased-rand}})
    \item We perform a design space exploration with \sysname's knobs across multiple datasets and find the knobs that achieve the best balance of performance and accuracy -- an average total training speedup of 1.8x (2.76x max) for an average 0.42\% point (1.79\% max) drop in final validation accuracy (\underline{Section~\ref{subsec:main-knob-sweep}})
    \item We show that with fixed hyperparameter tuning and training budgets, \sysname is able to train for more epochs and improve test accuracy (\underline{Section~\ref{subsec:hyperparam-tuning}})
    \item We show that \sysname offers additional improvements in the presence of a software-managed cache (\underline{Section~\ref{subsubsec:sw-gpu-cache}}) and when the problem size relative to the on-chip cache capacity grows (\underline{Section~\ref{subsec:l2-cache-sensitivity}})
\end{itemize}
%%

%\christos{One may start wondering how easy is it to navigate the continuum. how does the user know the right point to be operating one. It's nice to indicate that we have a suggestion that you get to eat a lot of your pie (but not all), while keeping it too. A default setting that many people will use.} \VB{Our latest round of results suggest that a particular combination of knobs seems to consistently achieve the highest total training time. Maybe we could call this out explicitly here? Haggai's suggestion below of discussing the per-epoch time vs number of epochs to converge would also help provide the intuition for these "best" knobs}

%\haggai{consider introducing the epoch time/num epochs tradeoff that our method reveals}

%% \begin{figure}[t]
%% \centering
%% \includegraphics[keepaspectratio,width=\columnwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/teaser-figure-perfonly.pdf}
%% \caption{{\bf Impact of community-structure biased randomized mini-batching on GNN training:}
%% {\em \sysname improves net training performance while achieving comparable accuracy (within XX\% points of the baseline)}
%% }
%% %\vspace{-2ex}
%% \label{fig:teaser-results}
%% \end{figure}


%% Using \sysname, we systematically explore the design space between random and structure-based mini-batching across four popular graph learning benchmarks to find the optimal balance between these approaches (Section~\ref{sec:eval}). 
%% %
%% Figure~\ref{fig:teaser-results} shows that \sysname, with optimized parameters, reduces total GNN training time by up to 1.9x (1.43x on average) compared to random mini-batching, while achieving comparable validation accuracy (within 0.7\% points).
%% %%

==> methodology.tex <==
\section{Experimental Methodology} \label{sec:methodology}

In this section, we provide details about the datasets, software, training methodology, and the platform used to evaluate the effectiveness of \sysname.
%%

{\bf Software and implementation: }
We perform all our evaluations on the NVIDIA NGC container~\cite{nvidia-dgl-container} of the Deep Graph Library (DGL)~\cite{wang2019deep} framework (v24.07).
%
We use DGL's in-built APIs for different neighborhood sampling schemes and extend the reference implementations of GraphSAGE and other GNN models.
%
Specifically, we implement the different root node partitioning schemes by creating appropriate permutations of the tensor containing the training set before passing it to DGL's DataLoader. 
%
%
To implement biased neighborhood sampling, we use DGL's NeighborSampler API that allows specifying the (unnormalized) probability of each edge in the graph~\cite{dgl-ngh-sampling} and then set the probability of all intra-community edges to $p$ and the probability of inter-community edges to $1-p$. 

\textbf{Evaluated schemes.} Table~\ref{table:root-mapping-policies} lists the root node partitioning policies we evaluate. 
%
For the \sysname knob for biased root partitioning, we represent the number of communities to mix ($k$) as a percentage of the total number of communities in the training set and evaluate 3 values of $k$ (12.5\%, 25\%, and 50\%).
%
We evaluate three values of $p$ for biased neighborhood sampling: $0.5$ (equal likelihood of sampling all edges in the graph), $0.9$ (the probability to sample a neighbor from the same community is $9$ times higher than a neighbor from another community), and $1.0$ (only sample neighbors from the same community).
\begin{table*}[ht]
\caption{{\bf Root node partitioning schemes evaluated}}
%% \caption{{\bf Root node mapping policies evaluated}\haggai{tables too small}\gal{Replace table with text? This part is important. }}
\label{table:root-mapping-policies}
\centering
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{ll}
\toprule
\textbf{Root Node Partitioning }   
& \textbf{Description}  \\ \midrule
RAND-ROOTS            & Uniform random shuffling of the training set before dividing nodes across batches  \\
NORAND-ROOTS         & No shuffling of the training set before dividing nodes across batches (root node partitioning is static across epochs) \\ 
COMM-RAND-MIX-0\%   & Shuffle communities as whole blocks; then shuffle contents within each community  \\ 
COMM-RAND-MIX-k\% & Shuffle communities as blocks; Combine fixed no. of communities (k\% of \#communities) into super-blocks; Shuffle within each super-block  \\ 
\bottomrule
\end{tabular}%
}
%\vspace{-2ex}
\end{table*}

{\bf Datasets: }
We evaluate \sysname across four graph datasets that are commonly used for evaluating GNNs (Table~\ref{table:datasets}).
%
The graphs used in our evaluation are diverse across multiple dimensions -- domains (social, citation, and product-purchasing networks), graph size (232K to 111M nodes), feature dimensions (100 to 1024), and training split (1\% to 65\% of nodes labeled).
%
For most of our evaluation, we assume that the graphs are already community-ordered because, in addition to powering \sysname, community-based reordering is an effective optimization for GNN inference as well (Section~\ref{sec:background}).
%
Only the uniform random mini-batching baseline for ClusterGCN comparisons (Section~\ref{subsec:prior-work-comparison}) runs on the original graph ordering.
%
We use RABBIT~\cite{rabbit} to perform community-based graph reordering and find the community membership of each node.
%
Section~\ref{subsec:preprocessing-cost} shows that reordering would impose negligible overhead.
%
As mentioned in Appendix B.4 of the OGB paper~\cite{ogb}, we use the symmetrized version of the {\tt ogbn-papers100M} dataset since the directed version leads to poor accuracy with GraphSAGE.
%%

\begin{table}[h]
    \caption{{\bf Graph Datasets}}
    \label{table:datasets}
    \centering
    %\scalebox{0.85}{
    \setlength{\tabcolsep}{2pt} %
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccccc}
    \toprule
    \textbf{Graph}  & \textbf{\#Nodes} & \textbf{\#Edges} & \textbf{\#Labels} & \textbf{\#Feat} & \textbf{Train-Val-Test \%} \\ \midrule
    reddit~\cite{reddit-dgl-dataset}          & 232,965          & 114,615,892      & 41                & 602             & 66-10-24                \\ %\hline
    igb-small~\cite{igb}       & 1,000,000        & 13,070,502       & 19                & 1024            & 60-20-20                \\ %\hline
    ogbn-products~\cite{ogb}   & 2,449,029        & 123,718,280      & 47                & 100             & 8-2-90                  \\ %\hline
    ogbn-papers100M~\cite{ogb} & 111,059,956      & 3,228,124,712    & 172               & 128             & 1.1-0.1-0.2             \\ 
    \bottomrule
    \end{tabular}%
    }
    %\vspace{-3ex}
\end{table}

{\bf Training methodology:}
%
Most of our evaluation focuses on training a 3-layer GraphSAGE model (we evaluate \sysname's impact on other GNN models in Section~\ref{subsec:other-gnn-models}).
%
For our evaluations, we perform training of up to 100 epochs (50 epochs for {\tt ogbn-papers100M} due to its size) with early-stopping.
%
We stop training if the validation loss does not improve for 6 epochs and measure the final validation accuracy after convergence.
%
Additionally, we also use PyTorch's {\em ReduceLROnPlateau} learning rate scheduler with default parameters and a patience of 3 epochs.
%
Training is performed on the default hyper-parameters used in the DGL's reference implementation of GraphSAGE (Batchsize=1024, fanout=10, learning rate=1e-3, weight decay=5e-4, and hidden dim=256). 
%
We calculate training metrics by averaging results across 5 random seeds (the same seeds are used for all configurations).
%%

%% \begin{table}[ht]
%%     \caption{{\bf Hyper-Parameters}\gal{Why spend space of a table on this? }}
%%     \label{table:hyperparams}
%%     \centering
%%     \resizebox{\columnwidth}{!}{%
%%     \begin{tabular}{ccccc}
%%     \toprule 
%%     \textbf{Batch Size} & \textbf{Fanout} & \textbf{Learning Rate} & \textbf{Weight Decay} & \textbf{Hidden Dim} \\
%%     \midrule
%%     1024                & (10, 10, 10)    & 1e-3                   & 5e-4                  & 256                \\
%%     \bottomrule
%%     \end{tabular}%
%%     }
%% \end{table}

{\bf Hardware platform: }
We perform our experiments on an NVIDIA Ampere A100 GPU with 80GB memory, 40MB of L2 cache, and 2039 GB/s of peak memory bandwidth.
%
A100's memory capacity allows us to store the graph and features on the GPU device memory for {\tt reddit}, {\tt ogbn-products}, and {\tt igb-small} datasets and, therefore, the training on these datasets is done purely on the GPU.
%
For {\tt ogbn-papers100M}, the graph and feature data are stored in pinned host (CPU) memory and DGL's dataloader uses Unified Virtual Addressing (UVA)~\cite{dgl-dataloader-api} to perform mixed CPU-GPU training.
%%


==> perfvsacc.tex <==
\section{Performance versus Accuracy Trade-off} \label{sec:perf-vs-acc} 

We will be evaluating the impact of biased mini-batch creation for two training scenarios -- (1) fixed number of epochs and (2) train until convergence. 
%
Studying the fixed number of epoch training scenario helps us understand the performance implications of biased mini-batch construction without worrying about differing rates of convergence. \christos{explain how you pick the fixed number of epochs. One natural selection is the number of epochs needed for convergence in the baseline. If you use something else, justify please}
%
This section shows results for the fixed-epoch training use-case.
%%

%%\subsection{Pareto-optimal curves}
\subsection{Runtime vs Accuracy curves}
\begin{itemize}
    \item Figure~\ref{fig:speedups-vs-acc-isoepochs} shows the iso-epoch training speedup vs validation accuracy trends.
\end{itemize}

\begin{figure*}[ht]
\centering
\includegraphics[keepaspectratio,width=\textwidth]{./Results/speedups-and-valacc_isoepochs_gpu-a100-sxm4-80gb.pdf}
\caption{{\bf Impact of biased mini-batch construction on runtime performance and accuracy}:
    {\em Results after 25 epochs of training. All results are normalized to the unbiased random baseline (Knob1=Uniform-Random + Knob2=50\%). As the likelihood of preferentially selecting intra-community neighbors increases (i.e. Knob-2), we see higher speedups. Compared to no randomization, community-aware randomization offers a good balance between total training speedup and final validation accuracy.\gal{Figure is intimidating. Replace bars with curves? }}
}
\label{fig:speedups-vs-acc-isoepochs}
\end{figure*}

\subsection{Reasons for performance improvements}
\haggai{this seems very important to me. If we can come up with some interesting explanations to what we see in the experiments that could be great}

\begin{itemize}
    \item Use this section to talk about how leveraging community structure improves reuse. Specifically, show how increasing the level of bias across two knobs reduces the input feature size (and brings it closer to the l2 capacity)
    \item To prove the above point, rely on NCU statistics and/or instrument how biased mini-batches affects size of the graphs (which allows analyzing footprint vs L2 capacity)
    \item The goal should be to explain how {\em both}  knob1 and knob2 impact feature size (and, therefore, speedup) \christos{also give reader an intuition about when to stop optimizing/turning knobs. When do you reach diminishing return in performance anyway due to X and Y hardware characteristics.}
\end{itemize}

\begin{figure}[ht]
\centering
\includegraphics[keepaspectratio,width=\columnwidth]{./Results/PerEpochTime_vs-batchstats-perepochonly_gpu-a100-sxm4-80gb.pdf}
\caption{{\bf Reasons for per-epoch speedup with biased mini-batch construction}:
    {\em Biased mini-batch construction policies require fetching fewer input features per batch. The per-epoch runtime is strongly correlated with the average size of the input feature vector across batches}
}
\label{fig:perepochtime-vs-featsize}
\end{figure}

\subsection{Reasons for accuracy loss}
\begin{itemize}
    \item The goal is to try and explain why the validation accuracy gap between baseline and biased mini-batch construction differs across datasets.
    \item Early results show that final accuracy is mostly correlated to average number of labels across mini-batches. 
    \item Mention that prior works showed that order of processing batches is important for accuracy too (and that different forms of randomization effectively reflect different batch processing orders)
    \item Come up with a metric that measures the divergence in labels among consecutive batches and show that randomizing root nodes trivially achieves that
    \item \VB{I wonder if we should even show results without Learning Rate scheduling at all (because it improves the baseline too)}
\end{itemize}

\subsection{Best solution?}
\begin{itemize}
    \item Use this section to summarize the performance and accuracy learnings from from previous subsections.  
    \item Give a teaser of other forms of biased randomization that will help bridge the accuracy gap
    \item Maybe this is also the section to discuss thoughts on how to find the best biased mini-batch construction approach for a given dataset.
    %\item Maybe this is also the section to discuss thoughts on finding the knob settings that can maximize performance gain for a given amount of accuracy loss (i.e. find points on the pareto-optimal curve) \haggai{sounds good. Do we aim to have experiments on that?}
\end{itemize}

==> rand-vs-structure.tex <==
%% \section{Randomization vs Structure-awareness in Mini-batching} \label{sec:rand-vs-structure}
\section{Tension between Randomization vs Structure-Awareness in Mini-Batching} \label{sec:rand-vs-structure}

In the previous section we discussed the use of randomization in mini-batch training of GNNs.
%
This section explores how graph structure and randomization create a trade-off between per-epoch training speed and overall training convergence (number of epochs until convergence).
%%

%\haggai{I would slightly change the structure of this section. my suggestion is to shape three bolded paragraphs: (1 )to first show what happens experimentally with pure structural mini batching; (2) then show what happens with pure randomization (3) discuss the pros and cons of each approach and motivate our method in the next section that combines both}
%
%\VB{I like the pure structural vs pure random framing. However, that might come at the expense of not being to focus on graph reordering for a subsection. I tried to incorporate the above framing while also giving the spotlight to reordering (since it is the basis for our optimization).}
\begin{figure}[t]
    \centering
    \includegraphics[keepaspectratio,width=0.85\columnwidth]{./Figures/rabbit-example.pdf}
\caption{{\bf Community-based Graph Reordering:} 
{\em Assigning community members consecutive IDs improves locality}
%{\em Reordering does not change the graph's structure. Instead, it only improves the sparsity pattern or data layout of the graph.}
}
%\vspace{-4.0ex}
\label{fig:reordering-example}
\end{figure}

{\bf Benefits of community-based graph reordering: } \label{subsec:graph-reordering} 
%
Real-world graphs exhibit strong structural properties (such as community structure~\cite{communities} and power-law degree distributions~\cite{powerlaw}) that can be leveraged to improve performance on graph-processing applications.
% 
Graph Reordering is one such optimization where the order of nodes in the graph is altered to reflect a graph structural property~\cite{rabbit,when-is-reordering-opt,cagra,rabbitpp-ispass2023,grasp-hpca20,gorder}.
%
Figure~\ref{fig:reordering-example} shows an example of a graph with random node ordering (left panel).
%
However, this graph exhibits community structure and reordering the nodes of the graph, such that members of a community have consecutive ordering, significantly improves the sparsity pattern of the graph post-reordering (right panel).
%%

%%
%Graph structure-aware reordering \haggai{add references}, a procedure in which the nodes in the graphs are reordered according to some structural property or measure (e.g., trying to minimize distances between subsequent nodes), is a well-established optimization technique in graph analytics and sparse linear algebra, traditionally used to improve memory locality and cache utilization. 
%
%\gal{has anyone tried this approach? If so, lets turn this into a more concrete and specific baseline.}
%%
%\VB{ClusterGCN uses a form of the above reordering. However, we will show later in the evaluation that it has certain fundamental limitations.}



Reordering improves performance of graph-based computations by primarily improving data reuse in on-chip caches.
%
The data footprint of typical graphs often far exceeds the limited cache capacity available in processors.
%
In an unordered graph (Figure~\ref{fig:reordering-example} left panel), the sparsity pattern leads to a highly irregular memory access pattern that often misses in the cache and requires performing expensive main-memory accesses.
%
In a community-reordered graph (right panel), the structured sparsity pattern means members of a community are likely to be accessed together which leads to high {\em spatial} and {\em temporal} locality.
%
Since the data footprint of communities are smaller than the entire graph, community-based reordering improves cache utilization and performance.
%%

{\bf Impact of reordering on GNN inference and training: }
%
Since GNN inference has a similar memory access pattern as traditional graph analytics workloads and inference accuracy is largely invariant to the node ordering, prior work has applied (community-based) graph reordering to GNN inference and achieved significant reductions in inference time~\cite{grow-hpca23,gnnadvisor-osdi21}.
%
Our experiments corroborate these findings and we observe that community-based reordering reduces the inference time of a GraphSAGE network by up to 26\% (12\% on average).
%
However, when applied to GraphSAGE {\em training}, reordering only improves training time by 3\% on average.
%
The lackluster improvement in GNN training is an artifact of randomization in mini-batch construction.
%
While essential for improving convergence (Section~\ref{sec:background}), randomization in mini-batching undoes the data reuse advantages of graph reordering\footnote{We note that graph reordering combined with full-batch training could potentially match the performance of standard mini-batching. However, this approach would still face all the limitations of full-batch training.}. 

%\haggai{this paragraph is a bit confusing to me. the main point made here is that structure can help computation on graphs, but randomness destroys structure and therefore just adding structure without accounting for randomness will not work. Questions: (1) is this what we want to say here? (2) if this is indeed what we want to say, I think we can write it in a more straight forward way and probably pick a better title for the paragraph. }
%%

%{\bf The need for randomization:} \haggai{consider changing this paragraph title as well to better reflect what we say here}
{\bf The cost of eliminating randomization: }
%
The reason why conventional mini-batch training is unable to benefit from graph reordering is because the randomization used during mini-batch construction is agnostic to the graph's structure (i.e. community structure).
%
Therefore, one possibility for improving mini-batch training performance would be to skip randomization during mini-batch construction.
%
Specifically, if we do not shuffle node IDs before partitioning the root nodes (Algorithm~\ref{alg:minibatch}; Line 2) and sample the $L$-hop neighborhood (Line 4) in a manner such that we always select neighbors belonging to the same community as the nodes within the batch, then we will have mini-batches that reflect the community structure of a reordered graph.
%
We compared such an entirely community-based mini-batch construction scheme against the uniform randomization used in conventional mini-batch training and Figure~\ref{fig:rand-vs-norand-extreme} shows results for training a GraphSAGE network on two datasets.
%
Skipping randomization allows community based mini-batching to benefit from data-reuse improvements of a reordered graph and reduces the per-epoch training time compared to uniform random mini-batching.
%
For the {\tt ogbn-papers100M} dataset, skipping randomization provides a per-epoch speedup of 4.5x which leads to a net training speedup of 2.7x in spite of taking 1.7x more epochs to converge.
%
However, entirely community-based mini-batching leads to a significant degradation in final validation accuracy by nearly 4\% points (Figure~\ref{fig:rand-vs-norand-extreme:ogbn-papers100M}).
%
For the {\tt reddit} dataset, while the accuracy loss is minor, the per-epoch speedup of 1.85x is insufficient to counter a delay in convergence by 2.17x epochs which causes the net training time to {\em increase} by 1.2x (Figure~\ref{fig:rand-vs-norand-extreme:reddit}).
%
The lack of randomization in an entirely community-based mini-batching results in poor quality mini-batches (low diversity within batches) which impacts convergence and accuracy. 
%%

%% \begin{figure}[t]
%%     \centering
%%     \includegraphics[keepaspectratio,width=\columnwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/rand-vs-norand-extremes.pdf}
%%     \caption{{\bf Impact of eliminating randomization from mini-batching:}
%%     {\em Per-epoch time improves by XX but accuracy drops by XX\% points and total training time increases by XX}
%%     }
%%     %\vspace{-3ex}
%%     \label{fig:rand-vs-norand-extreme}
%% \end{figure}

\begin{figure}[ht]
    \centering
    \begin{subfigure}[]{0.49\columnwidth}
        \centering
        \includegraphics[keepaspectratio,width=\columnwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/rand-vs-norand-extremes-v2_graph-ogbn-papers100M-symm.pdf}
        \caption{ogbn-papers100M}
        \label{fig:rand-vs-norand-extreme:ogbn-papers100M}
    \end{subfigure}
    \hfill
    \begin{subfigure}[]{0.49\columnwidth}
        \centering
        \includegraphics[keepaspectratio,width=\columnwidth]{GNN-Biased-Minibatching-MLSys-2025-Draft/Results/rand-vs-norand-extremes-v2_graph-reddit.pdf}
        \caption{reddit}
        \label{fig:rand-vs-norand-extreme:reddit}
    \end{subfigure}
    \caption{{\bf Impact of entirely community-based mini-batching:}
    {\em Removing randomization leads to (a) accuracy loss and/or (b) a net training slowdown due to delayed convergence}
    }
    %\vspace{-3ex}
    \label{fig:rand-vs-norand-extreme}
\end{figure}

{\bf Conclusion: }
%
The above results highlight a fundamental tension between randomization vs leveraging graph structure in mini-batching.
%
Ignoring graph structure (i.e. uniform random mini-batching) misses an opportunity to optimize per-epoch training time while completely ignoring randomization (entirely community-based mini-batching) comes at the expense of accuracy loss and delayed convergence.
%%

%The result highlights a fundamental tension: randomization in the training procedure is crucial for improving convergence (Figure~\ref{fig:full-vs-mini-batch}) but this randomization comes at the expense of not being able to leverage the benefits of structure within graphs



==> related.tex <==
\section{Related Work} \label{sec:related}

We discussed prior work on GNN mini-batching in Sections~\ref{sec:background} and ~\ref{subsec:prior-work-comparison}. In this section, we compare \sysname against general GNN training and inference optimizations.
%%

Merkel et. al.~\cite{can-reordering-speedup-gnn-training-vldb24} performed an extensive study of the impact of different reordering techniques (including RABBIT) on GNN training.
%
However, their work largely focused on full-graph training (which has slower convergence vs mini-batch training; Section~\ref{sec:background}) and does not explore reordering's impact on training accuracy (which can be quite severe as shown in Figure~\ref{fig:rand-vs-norand-extreme:ogbn-papers100M}).
%
Similarly, Neugraph~\cite{neugraph-atc19} and ROC~\cite{roc-mlsys20} target the scalability challenges of full-graph GNN training.
%
SALIENT~\cite{salient-mlsys22} improves mini-batch GNN training and inference performance by pipelining the batch creation (on CPU) and data transfer steps with the training computations (on GPU) to maximize GPU utilization.
%
\sysname reduces the size of each batch's subgraph and, therefore, can help SALIENT's pipelining by saturating GPU utilization with fewer CPU processes.
%
Betty~\cite{betty-asplos23} proposed a partitioning strategy to sub-divide mini-batches into micro-batches in order to scale GNN training to larger graph sizes.
%
Betty maximizes memory savings by reducing redundancy across the micro-batches and \sysname's community-biased mini-batches are likely to help with finding low redundancy partitions (as shown in Figure~\ref{fig:biased-ngh-selection}).
%
There have been many GNN accelerator proposals~\cite{hygcn-hpca20,awb-gcn-micro20,grow-hpca23,igcn-micro21} but they primarily target GNN inference.
%
GNN inference typically operates on the entire graph and is invariant to the order in which nodes are processed (and therefore benefits from graph reordering optimization).
%
In contrast, mini-batch GNN training exhibits a more challenging access pattern where the number of nodes processed is a function of the training set of the graph and the need for randomization leads to a very dynamic reuse pattern that changes each training epoch.
%%



